ScionFL: Efficient and Robust Secure Quantized Aggregation

Secure aggregation is commonly used in federated learning (FL) to alleviate privacy concerns related to the central aggregator seeing all parameter updates in the clear. Unfortunately, most existing secure aggregation schemes ignore two critical orthogonal research directions that aim to (i) significantly reduce client-server communication and (ii) mitigate the impact of malicious clients. However, both of these additional properties are essential to facilitate cross-device FL with thousands or even millions of (mobile) participants. In this paper, we unite both research directions by introducing ScionFL, the first secure aggregation framework for FL that operates efficiently on quantized inputs and simultaneously provides robustness against malicious clients. Our framework leverages (novel) multi-party computation (MPC) techniques and supports multiple linear (1-bit) quantization schemes, including ones that utilize the randomized Hadamard transform and Kashin's representation. Our theoretical results are supported by extensive evaluations. We show that with no overhead for clients and moderate overhead for the server compared to transferring and processing quantized updates in plaintext, we obtain comparable accuracy for standard FL benchmarks. Moreover, we demonstrate the robustness of our framework against state-of-the-art poisoning attacks.

==> Sections_ScionFL/4_Our_System.tex <==
In this section, we present our system \FLname{} in detail from an~MPC standpoint.
We present the underlying sharing semantics, client interaction with~MPC servers, and methods for performing secure aggregation of client updates.
We begin by introducing the masked evaluation technique, which is used to improve our system's real-time performance.

%----------------------------------------
\tsparagraph{Masked Evaluation}
\label{sec:masked_evaluation}
%----------------------------------------
In our~MPC protocols, we use the masked evaluation technique~\cite{AC:GorRanWan18,ACNS:BenNieOmr19,ndss:ChaudhariRS20,USENIX:MLRG20,ARXIV:MPCLeague,EPRINT:KPPS22}, which enables the costly~\emph{data-independent} calculations to be completed in a preprocessing phase, thus enabling a fast and efficient~\emph{data-dependent} online phase~(cf.~\secref{sec:prelims_mpc}). 
%
In this model, the secret-share of every element~$\val \in \Z{\ell}$, denoted by~$\shr{\val}$, is associated with two values: a random mask~$\lv{\val}{} \in \Z{\ell}$ and a masked value~$\mv{\val} \in \Z{\ell}$ such that~$\val = \mv{\val} + \lv{\val}{}$.
While~$\lv{\val}{}$ is split and distributed as~$\numshares$ shares similar to the general case discussed in~\secref{sec:approx-bit-arithmetic}, $\mv{\val}$ is given to all~MPC servers\footnote{Due to differences in the underlying setting, there may be minor differences in how the values~$\mv{\val}$ and~$\lv{\val}{}$ are distributed among the servers.}.
Since~$\lv{\val}{}$ is random and independent of~$\val$, all operations involving~$\lv{\val}{}$ values alone can be computed during the preprocessing phase.

%----------------------------------------
\tsparagraph{Masked Bit Conversion and Injection}
%----------------------------------------
%
With the masked evaluation technique, the arithmetic equivalent~$\bitbext$ for a bit~$\bitb =  \mv{\bitb} \xor \lv{\bitb}{}$ can be obtained as 
%
\begin{align}
\label{eq:case-bitA-masked}
\bitbext = \mv{\bitb} \xor \lv{\bitb}{} = \Mv{\bitb} + (1 - 2\mv{\bitb}) \cdot \Lv{\bitb}{},
\end{align}
%
where~$\Mv{\val}$ and~$\Lv{\val}{}$ denote the arithmetic equivalents of~$\mv{\val}$ and~$\lv{\val}{}$, respectively.
Note that~$\Lv{\bitb}{}$ can be computed from~$\lv{\bitb}{}$ during the preprocessing phase using techniques discussed in~\secref{sec:approx-bit-arithmetic}, including our novel approximation from \secref{sec:our-approx}.
Similarly, given~$\scale = \Mv{\scale} + \Lv{\scale}{}$, the value~$\bitb \cdot \scale$ can be obtained as
%
\begin{small}
\begin{align}
\label{eq:case-bitinj-masked}
    \bitb \cdot \scale &= (\Mv{\bitb} + (1 - 2\mv{\bitb}) \cdot \Lv{\bitb}{}) \cdot (\Mv{\scale} + \Lv{\scale}{}) \nonumber \\
    &= \Mv{\bitb}\Mv{\scale} + \Mv{\bitb} \Lv{\scale}{} + (1 - 2\mv{\bitb}) \cdot (\Lv{\bitb}{} \Mv{\scale} +  \Lv{\bitb}{}\Lv{\scale}{}).
\end{align}
\end{small}
%
As shown in~Eq.~\eqref{eq:case-bitinj-masked}, the servers need to additionally compute~$\Lv{\bitb}{}\Lv{\scale}{}$ in the preprocessing phase. 

%----------------------------------------
\tsparagraph{Client Interaction}
\label{sec:client-interaction}
%----------------------------------------
Before going into the details of aggregation among the~$\numservers$~MPC servers, we discuss input sharing and the reconstruction of the aggregated vector for clients.

To generate the~$\shr{\cdot}$-shares of a value~$\val \in \Z{\ell}$ owned by client~$\client{}$, it first non-interactively computes the additive shares of the mask~$\lv{\val}{}$ using the shared randomness setup discussed in~\secref{sec:mpc-shared-randomness}.
The masked value is then computed as~$\mv{\val} = \val - \lv{\val}{}$ and sent to a single designated~MPC server, say~$\server{1}$.
The input sharing is completed when~$\server{1}$ sends~$\mv{\val}$ to all remaining MPC servers.
%
For~Boolean values~(i.e., $\Z{}$) the procedure is similar except that addition/subtraction is replaced with~XOR and multiplication with~AND.
We use~$\shrB{\cdot}$ to denote the secret sharing over the domain~$\Z{}$.

After the servers have received all inputs in~$\shr{\cdot}$-shared form, they instantiate the~$\FSecAgg$ functionality specified in~\boxref{fig:secure-aggregation-accurate} and obtain the aggregated vectors in~$\shr{\cdot}$-shared form.
%
Recall from~\secref{sec:fl-aggregation} that the values to be aggregated in our case correspond to~FL gradients, and the aggregated result can also be made public.
%
As a result, the servers reconstruct the aggregated result towards a chosen server, say~$\server{1}$, which updates the global model according to~Eq.~\eqref{eq:fedavg}. In the next iteration, $\server{1}$ distributes the updated global model to a fresh set of clients, and the process is repeated.

From a client's perspective, it is only interacting with one server~(apart from a one-time shared-randomness setup), as it is the case in a privacy-free variant in which clients communicate with a single parameter server for aggregation~\cite{PMLR:McMahanMRHA17}.

\tsparagraph{MPC Protocols}
%
We provide the full~MPC protocols for inner product computation, multiplication, and bit-to-arithmetic conversion in~\appref{app:mpc-protocols}, which are utilized in a black-box fashion in this section.

%%---------------------------------------%%
\subsection{MPC-based Aggregation}
\label{sec:mpc-agg}
%%---------------------------------------%%
We now discuss two approaches for instantiating~$\FSecAgg$ using~MPC protocols that operate on secret-shared values.
Recall from~Eq.~\eqref{eq:quantized-aggregation} that the~MPC servers for the aggregation of quantized values possess~$\shr{\cdot}$-shares of matrices~$\matD{U}{\numclients}{1}$ and~$\matD{V}{\numclients}{1}$ along with the~$\shrB{\cdot}$-shares of~$\matD{B}{\numclients}{\numcoordinates}$.

%----------------------------------------
\subsubsection{Approach I}
\label{sec:approach_I}
%----------------------------------------
A naive instantiation of~$\FSecAgg$ would be to have the servers convert binary shares of the matrix~$\mat{B}$ to their arithmetic shares first, as in~Prio+~\cite{SCN:AddankiGJOP22}.
This is possible in~MPC with a bit-to-arithmetic conversion protocol ~\cite{CCS:MohRin18,NDSS:PatSur20,SCN:AddankiGJOP22,EPRINT:KPPS22}, denoted by~$\piBitA$, which computes the arithmetic shares of~$\bitb \in \Z{}$ from its~Boolean sharing.
%
Once the arithmetic shares are generated, the servers use an instance of an inner-product protocol, denoted by~$\piDotP$, on each of the~$\numcoordinates$ columns of matrix~$\mat{B}$ with the column vector~$(\matD{V}{\numclients}{1} - \matD{U}{\numclients}{1})$ computed locally to obtain the row aggregate. 
%
They complete the protocol by adding a row aggregate of~$\mat{U}$ to each column of the resultant matrix computed in the previous step.
The formal protocol~$\piSecAgg{1}$ is given in~\boxref{fig:SecAgg-MPC-Approach-I}. 

\begin{protocolbox}{$\piSecAgg{1} (\shrB{\matD{B}{\numclients}{\numcoordinates}}, \shr{\matD{U}{\numclients}{1}}, \shr{\matD{V}{\numclients}{1}})$}{Secure aggregation -- Approach \Romannum{1}.}{fig:SecAgg-MPC-Approach-I}
	%----
	\justify
	\begin{description}
	    %-----
		\item[1.] Locally compute $\shr{\matD{S}{\numclients}{1}} = \shr{\matD{V}{\numclients}{1}} - \shr{\matD{U}{\numclients}{1}}$.
		%-----
		\item[2.] Compute $\shr{\mat{B}} = \piBitA(\shrB{\mat{B}})$.
		%-----
		\item[3.] Compute $\shr{\matcol{W}{j}} = \piDotP(\shr{\matcol{B}{j}},\shr{\mat{D}})$, for each $j \in [\numcoordinates]$.
		%-----
		\item[4.] Locally compute $\shr{\matD{Z}{1}{1}} = \rowAggregate(\shr{\matD{U}{\numclients}{1}})$.
		%-----
		\item[5.] Locally compute $\shr{\matD{Y}{1}{\numcoordinates}} = \shr{\matD{Z}{1}{1}} \oplus \shr{\matD{W}{1}{\numcoordinates}}$. 
		%-----
	\end{description} 
\end{protocolbox}



As shown in~\boxref{fig:SecAgg-MPC-Approach-I}, $\piSecAgg{1}$ invokes~$\piBitA$ for each bit in matrix~$\mat{B}$, resulting in~$\numclients\cdot\numcoordinates$ invocations. 
%
Using the masked evaluation technique~\cite{NDSS:KPRS22,ARXIV:MPCLeague}, the online communication of this approach can be made independent of the dimension~$\numclients$, which in our case corresponds to the number of clients.
%The details for this are discussed next.

%----------------------------------------
\subsubsection{Approach II}
\label{sec:approach_II}
%----------------------------------------
We use the bit injection protocol~\cite{CCS:MohRin18,NDSS:PatSur20,USENIX:KPPS21}, denoted by~$\piBitInj$, which computes the arithmetic sharing of~$\bitb\cdot\scale$ given the~Boolean sharing of~$\bitb \in \Z{}$ and the arithmetic sharing of~$\scale \in \Z{\ell}$.
%
Given~$\shrB{\matD{M}{\alpha}{1}}$ and~$\shr{\matD{N}{\alpha}{1}}$, the high-level idea is to effectively combine the~$\piBitA$ and~$\piDotP$ protocol to a slightly modified instance of~$\piBitInj$ that directly computes the sum~\cite{NDSS:KPRS22,ARXIV:MPCLeague}~(denoted by~$\sum_{i=1}^{\alpha} \matpos{M}{i}{1} \cdot \matpos{N}{i}{1}$) instead of the individual positions. This can be achieved following~Eq.~\eqref{eq:case-bitinj-masked} and the details appear in~\boxref{fig:bitinj-sum} in~\secref{app:mpc-protocols}. One significant advantage of this technique is that online communication is no longer dependent on the number of clients $\numclients$.
%
$\piSecAgg{2}$ denotes the resulting protocol and the formal details are given in~\boxref{fig:SecAgg-MPC-Approach-II}.


\begin{protocolbox}{$\piSecAgg{2} (\shrB{\matD{B}{\numclients}{\numcoordinates}}, \shr{\matD{U}{\numclients}{1}}, \shr{\matD{V}{\numclients}{1}})$}{Secure aggregation -- Approach \Romannum{2}.}{fig:SecAgg-MPC-Approach-II}
	%----
	\justify
	\begin{description}
	    %-----
		\item[1.] Locally compute $\shr{\matD{S}{\numclients}{1}} = \shr{\matD{V}{\numclients}{1}} - \shr{\matD{U}{\numclients}{1}}$.
		%-----
		\item[2.] Compute $\shr{\matcol{W}{j}} = \piBitInj(\shrB{\matcol{B}{j}},\shr{\mat{D}})$, for each $j \in [\numcoordinates]$.
		%-----
		\item[3.] Locally compute $\shr{\matD{Z}{1}{1}} = \rowAggregate(\shr{\matD{U}{\numclients}{1}})$.
		%-----
		\item[4.] Locally compute $\shr{\matD{Y}{1}{\numcoordinates}} = \shr{\matD{Z}{1}{1}} \oplus \shr{\matD{W}{1}{\numcoordinates}}$. 
		%-----
	\end{description} 
\end{protocolbox}



%----------------------------------------
\subsubsection{Approach III using SepAgg}
\label{sec:SepAgg}
%----------------------------------------
In a closely related work~\cite{ARXIV:BAT20}, the authors combine the~SIGNSGD compression technique of~\cite{ICML:BernsteinWAA18} with additive secret sharing for~FL.
Unlike our work, which investigates secure aggregation using various linear quantization algorithms in a cross-device environment, they aim for a cross-silo setting in which clients distribute arithmetically shared values to servers rather than single bits.
In terms of client-server communication, this indicates an overhead of factor~$\log_2 2\numclients$, where~$\numclients$ is the number of involved participants each round.

However, the authors of~\cite{ARXIV:BAT20} introduce an interesting approximation called~\enquote{SepAgg} for computing the averaged inner product between bits and scales:
\begin{equation}
    \label{eq:sepagg}
    \frac{1}{\numclients} \sum_i^\numclients \qvecV{X}{i} \cdot \stepV{X}{i} \approx \frac{1}{\numclients^2} \left(\sum_i^\numclients \qvecV{X}{i}\right) \left(\sum_i^\numclients \stepV{X}{i}\right).
\end{equation}

We adopt the~SepAgg method to our setting to compute~$\rowAggregate(\mat{B} \circ (\mat{V} - \mat{U}))$ in~Eq.~\eqref{eq:quantized-aggregation}.
In particular, we aggregate the matrices~$\mat{B}$ and~$(\mat{V}-\mat{U})$ independently and then perform one secure multiplication per coordinate, with the other operations being linear and free in our~MPC protocol.
As a result, we can utilize linear quantization schemes with local scales at the cost of global scales~(ignoring the overhead for global scales to securely determine~\stepmin{X} and~\stepmin{X} across all participants).
The formal protocol~$\piSecAgg{3}$ utilizing~SepAgg appears in~\boxref{fig:SecAgg-MPC-Approach-III}.

\begin{protocolbox}{$\piSecAgg{3} (\shrB{\matD{B}{\numclients}{\numcoordinates}}, \shr{\matD{U}{\numclients}{1}}, \shr{\matD{V}{\numclients}{1}})$}{Secure aggregation -- Approach \Romannum{3} (SepAgg~\cite{ARXIV:BAT20}).}{fig:SecAgg-MPC-Approach-III}
	%----
	\justify
	\begin{description}
	    %-----
		\item[1.] Locally compute $\shr{\matD{S}{1}{1}} = \rowAggregate(\shr{\matD{V}{\numclients}{1}} - \shr{\matD{U}{\numclients}{1}})$.
		%-----
		\item[2.] Compute $\shr{\matcol{T}{j}} = \piBitASum(\shrB{\matcol{B}{j}})$, for each $j \in [\numcoordinates]$.
		%-----
		\item[3.] Compute $\shr{\matcol{W}{j}} = \piMult(\shr{\matcol{T}{j}},\shr{\mat{S}})$, for each $j \in [\numcoordinates]$.
		%-----
		\item[4.] Locally compute $\shr{\matD{Z}{1}{1}} = \rowAggregate(\shr{\matD{U}{\numclients}{1}})$.
		%-----
		\item[5.] Locally compute $\shr{\matD{Y}{1}{\numcoordinates}} = \shr{\matD{Z}{1}{1}} \oplus \frac{1}{\numclients} \cdot \shr{\matD{W}{1}{\numcoordinates}}$. 
		%-----
	\end{description} 
\end{protocolbox}

%-------------------------------------
\tsparagraph{Accuracy Evaluation}
\label{sec:sepagg_eval}
%-------------------------------------
We next provide strong empirical evidence that applying~SepAgg for~SQ with preprocessing preserves the linear~NMSE decay with respect to the number of clients~(i.e., unbiased estimates).
For this, we run a simulation similar to the one described in~\secref{sec:approx_evaluation}.
Here, we compare the~NMSE computed as in~Eq.~\eqref{eq:nmse} for an aggregation~$\textit{agg}$~(1)~a regular dot product between converted bits and scales and~(2) with~SepAgg.
Note that here we do not apply our approximate conversion presented in~\secref{sec:approx-bit-arithmetic} to study the effect of~SepAgg in isolation.
Our results shown in~Fig.~\ref{fig:sepagg_sq} are the average of~10 trials for each experiment.
While for smaller vector dimensions, we observe a visible effect for~SQ without preprocessing, there is only a minor difference for the other two quantization schemes, and sometimes the~NMSE for~SepAgg is even smaller than for the exact computation.

\begin{figure}[htb]
    \centering
    \input{Figures/SepAgg_new}
    \vspace{-3mm}
    \captionsetup{font=small}
    \caption{NMSE comparison between exact and~SepAgg-based aggregation for vanilla~SQ, SQ using the randomized~Hadamard transform~(HSQ), and~SQ using~Kashin's representation~(KSQ) for various vector dimensions~$d$ and number of clients~$\numclients$.}
    \label{fig:sepagg_sq}
\end{figure}

Formally proving that applying~SepAgg after different preprocessing techniques, such as random rotation and Kashin's representation, results in an unbiased aggregation is a significant theoretical challenge. We leave this intriguing endeavor for future work.

\tsparagraph{Communication Costs}
%
We provide a detailed analysis of theoretical and concrete communication costs for each of our three approaches outlined in~\secref{sec:approach_I} to~\secref{sec:SepAgg} in~\appref{sec:communication_costs_detailed}.





==> preamble.tex <==
\usepackage{algorithm}
\usepackage{algpseudocode} 
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage[affil-it]{authblk}
\usepackage{booktabs}       % professional-quality tables
\usepackage{caption}
\usepackage{colortbl} %rowcolours
\usepackage{csquotes}
\usepackage{comment}
\usepackage{dsfont}
\usepackage{tablefootnote}
\usepackage{threeparttable}
\usepackage{graphicx}
\usepackage{pifont}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{mathtools}
\usepackage[framemethod=tikz]{mdframed} %For new boxes
\usepackage{multirow}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{orcidlink}
%For new boxes
\usepackage{ragged2e}
\usepackage{romannum} %Roman Numerals
\AtBeginDocument{\pagenumbering{arabic}}
%\usepackage{siunitx}
\usepackage{thmtools, thm-restate}
\usepackage{todonotes}
\usepackage[normalem]{ulem}
\usepackage{url}            % simple URL typesetting
\usepackage{xcolor}         % colors
\usepackage{xspace}

\usepackage{pgfplots}
\pgfplotsset{compat=1.15}

\usepackage{filecontents}
\usepackage{enumitem}

\usetikzlibrary{positioning}
\usepackage[draft]{tikzpeople}
\usetikzlibrary{arrows}
\usetikzlibrary{matrix}


\makeatletter
\tikzset{
    database/.style={
        path picture={
            \draw (0, 1.5*\database@segmentheight) circle [x radius=\database@radius,y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius, 0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius,-0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius,1.5*\database@segmentheight) -- ++(0,-3*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius] -- ++(0,3*\database@segmentheight);
        },
        minimum width=2*\database@radius + \pgflinewidth,
        minimum height=3*\database@segmentheight + 2*\database@aspectratio*\database@radius + \pgflinewidth,
    },
    database segment height/.store in=\database@segmentheight,
    database radius/.store in=\database@radius,
    database aspect ratio/.store in=\database@aspectratio,
    database segment height=0.1cm,
    database radius=0.25cm,
    database aspect ratio=0.35,
}
\makeatother

\usepackage[compact]{titlesec}


==> symbols.tex <==
%--------------------------------------------------------------
% Packages
%--------------------------------------------------------------
\IEEEoverridecommandlockouts

\makeatletter
\def\thanks#1{\protected@xdef\@thanks{\@thanks
        \protect\footnotetext{#1}}}
\makeatother

\makeatletter
\renewcommand\footnoterule{\relax\kern-5pt
\hrule
\kern4.6pt}
\makeatother

\input{preamble}

\newcommand{\FLname}{ScionFL\xspace}
\newcommand{\FLdefensename}{ScionFL-Aura\xspace}

\let\paragraphS\S
\let\oldS\S
\let\orgautoref\autoref
\renewcommand{\autoref}
{\def\equationautorefname{Equation}%
	\def\figureautorefname{Fig.}%
	\def\subfigureautorefname{Fig.}%
	\def\Itemautorefname{Item}%
	\def\tableautorefname{Tab.}%
	\def\algorithmautorefname{Alg.}%
	\def\paragraphautorefname{Paragraph}%
	\def\sectionautorefname{\oldS}%
	\def\subsectionautorefname{\oldS}%
	\def\subsubsectionautorefname{\oldS}%
	\def\appendixautorefname{App.\xspace}%
	\defhapterautorefname{Chapter}%
	\def\partautorefname{Part}%
	\def\goalautorefname{Goal}%
	\def\reqautorefname{Req.}%
	\def\adviceautorefname{Rule}%
	\def\parameterautorefname{Param.}%
	\def\definitionautorefname{Definition}%
	\def\theoremautorefname{Theorem}%
	\orgautoref}


%--------------------------------------------------------------
% Selection Control
%--------------------------------------------------------------
\newif\ifsubmission
\submissionfalse % editing (draft) version
%\submissiontrue % submission version

\newif\iffullversion
\fullversionfalse % proceedings version
\fullversiontrue % full version (ePrint)

\newif\ifanonymous
%\anonymousfalse % show author names
\anonymoustrue % hide author names & all identifying info

%--------------------------------------------------------------
% Macros for Colors
%--------------------------------------------------------------
\definecolor{darkred}{rgb}{.6,0,0}
\definecolor{darkgreen}{rgb}{0,.4,0}
\definecolor{darkblue}{rgb}{0,0,.6}
\definecolor{absolutezero}{rgb}{0.0,0.28,0.73}
\definecolor{acidgreen}{rgb}{0.69,0.75,0.1}
\definecolor{amazon}{rgb}{0.23,0.48,0.34}
\definecolor{ambersaeece}{rgb}{1.0,0.49,0.0}
\definecolor{antiquebronze}{rgb}{0.4,0.36,0.12}
\definecolor{aoenglish}{rgb}{0.0,0.5,0.0}
\definecolor{brightmaroon}{rgb}{0.76,0.13,0.28}
\definecolor{cadmiumred}{rgb}{0.89,0.0,0.13}
\definecolor{britishracinggreen}{rgb}{0.0,0.26,0.15}
\definecolor{lightgray}{gray}{0.9}

%--------------------------------------------------------------
% Macros for Layout/Structure
%--------------------------------------------------------------
\newcommand{\sect}[1]{§\ref{#1}} 
\newcommand{\prot}[1]{Prot.~\ref{#1}}

\newcommand{\secref}[1]{\S\ref{#1}}
%\newcommand{\appref}[1]{App.~\secref{#1}}
\newcommand{\appref}[1]{\secref{#1}}
%\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\newcommand{\tabref}[1]{Tab.~\ref{#1}}
%\newcommand{\algref}[1]{Alg.~\ref{#1}}

\newcommand{\makeparafit}{\looseness=-1}
\newcommand{\Mod}[1]{\ \mathrm{mod}\ #1}
%--------------------------------------------------------------
% Macros for Operators
%--------------------------------------------------------------
\newcommand{\xor}{\oplus}
\newcommand{\Xor}{\bigoplus}
\newcommand{\band}{\odot}
\newcommand{\bAnd}{\bigodot}
\newcommand{\booland}{\circledast}
\newcommand{\Order}{\mathcal{O}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\left(#1\right)}}
\newcommand{\defined}{\ensuremath{\stackrel{def}{=} }}
\newcommand{\iseq}{\ensuremath{\stackrel{?}{=} }}

\newcommand{\invcircledast}{%
  \mathbin{\vphantom{\circledast}\text{%
    \ooalign{\smash{\blackcircle}\cr
             \hidewidth\smash{\textcolor{white}{$*$}}\hidewidth\cr
            }%
  }}%
}
\newcommand{\invodot}{%
  \mathbin{\vphantom{\odot}\text{%
    \ooalign{\smash{\blackcircle}\cr
             \hidewidth\smash{\whitedot}\hidewidth\cr
            }%
  }}%
}

\newcommand{\blackcircle}{\raisebox{-.4ex}{\scalebox{1.66}{$\bullet$}}}
\newcommand{\whitedot}{\raisebox{.4ex}{\textcolor{white}{\scalebox{.3}{$\bullet$}}}}

\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\ceil}[1]{\lceil#1\rceil}

%--------------------------------------------------------------
% Fields vs Rings
%--------------------------------------------------------------
\newcommand{\FF}{\mathbb{F}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}

%--------------------------------------------------------------
% Macros for ML Part
%--------------------------------------------------------------
\newcommand{\dimension}{\ensuremath{\mathsf{m}}}
\newcommand{\numOne}{\ensuremath{N_\mathsf{one}}}
\newcommand{\numZero}{\ensuremath{N_\mathsf{zero}}}

\newcommand{\lone}[1]{\ensuremath{\mathsf{L1}~(#1)}}
\newcommand{\ltwo}[1]{\ensuremath{\mathsf{L2}~(#1)}}


%--------------------------------------------------------------
% General Notations
%--------------------------------------------------------------
%Matrices
\newcommand{\mat}[1]{\ensuremath{\vec{\mathbf{#1}}}}
\newcommand{\matD}[3]{\ensuremath{\vec{\mathbf{#1}}_{\sf#2\times#3}}}
\newcommand{\matrow}[2]{\ensuremath{\vec{\mathbf{#1}}_{#2}}}
\newcommand{\matcol}[2]{\ensuremath{\vec{\mathbf{#1}}^{#2}}}
\newcommand{\matpos}[3]{\ensuremath{{\mathbf{#1}}_{#2}^{#3}}}

%Quantization
\newcommand{\qvec}[1]{\ensuremath{\vec{\sigma}_{#1}}}
\newcommand{\qvecV}[2]{\ensuremath{\vec{\sigma}_{#1}^{#2}}}
\newcommand{\stepV}[2]{\ensuremath{\vec{\mathsf{s}}_{#1}^{#2}}}
\newcommand{\stepmin}[1]{\ensuremath{\mathsf{s}_{#1}^{min}}} 
\newcommand{\stepmax}[1]{\ensuremath{\mathsf{s}_{#1}^{max}}} 
\newcommand{\vecq}[1]{\ensuremath{\vec{{#1}}_{\sigma}}}
\newcommand{\vecqV}[2]{\ensuremath{\vec{{#1}}_{\sigma}^{#2}}}

%Aggregation
\newcommand{\rowAggregate}{{\sf Agg\mbox{-}R}}
\newcommand{\colAggregate}{{\sf Agg\mbox{-}C}}

%Defense
%\newcommand{\aggvec}{\ensuremath{\vec{\Gamma}}}
\newcommand{\aggvec}{\ensuremath{\vec{X}}}
\newcommand{\aggvecD}[2]{\ensuremath{\vec{\aggvec}_{\sf#1\times#2}}}
\newcommand{\aggFull}{\ensuremath{\aggvec^{\sf agg}}}
\newcommand{\aggDef}{\ensuremath{\aggvec^{\sf aggd}}}

%--------------------------------------------------------------
% Macros for ideal functionalities
%--------------------------------------------------------------
\newcommand{\Funct}[1]{\ensuremath{\mathcal{F}_{\mathsf{#1}}}}
\newcommand{\FHWeight}{\ensuremath{\mathcal{F}_{\mathsf{hweight}}}}
\newcommand{\FHWeightApprox}{\ensuremath{\mathcal{F}_{\mathsf{hweight}}^{\mathsf{approx}}}}


\newcommand{\FSecAgg}{\ensuremath{\mathcal{F}_{\mathsf{SecAgg}}}}
\newcommand{\Adv}{\ensuremath{\mathcal{A}}}

\newcommand{\FSecAggE}{\ensuremath{\mathcal{F}_{\mathsf{SecAgg}}^{\mathsf{apx}}}}

%--------------------------------------------------------------
% Macros for Secure Aggregation
%--------------------------------------------------------------
\newcommand{\approxFactor}{\ensuremath{\mathcal{E}}}

\newcommand{\bitvector}[1]{\ensuremath{\vec{\mathsf{b}^{#1}}}}
\newcommand{\bitV}[2]{\ensuremath{\mathsf{b}^{#1}_{#2}}}
\newcommand{\bitVext}[2]{\ensuremath{\tilde{\mathsf{b}}^{#1}_{#2}}}
\newcommand{\scaleV}[1]{\ensuremath{\mathsf{s}^{#1}}} 

\newcommand{\aggvector}{\ensuremath{\vec{\mathsf{y}}}}
\newcommand{\aggV}[1]{\ensuremath{\mathsf{y}_{#1}}}

\newcommand{\samplesize}{\ensuremath{\mathsf{p}}}
\newcommand{\sampleset}{\ensuremath{\mathcal{I}}}
\newcommand{\sampleindex}[1]{\ensuremath{\mathsf{ind}_{#1}}}





%--------------------------------------------------------------
% Macros for Values
%--------------------------------------------------------------
\newcommand{\vecbit}{\ensuremath{\mathsf{b}}}
\newcommand{\vbitv}[1]{\ensuremath{\mathsf{b}_{#1}}} 
\newcommand{\vbits}[2]{\ensuremath{\mathsf{b}_{#1,#2}}} 

%Arithmetic equivalent
\newcommand{\arvecbit}{\ensuremath{\mathsf{b}^{\sf A}}}
\newcommand{\arvbitv}[1]{\ensuremath{\mathsf{b}_{#1}^{\sf A}}} 
\newcommand{\arvbits}[2]{\ensuremath{\mathsf{b}_{#1,#2}^{\sf A}}} 

\newcommand{\scale}{\ensuremath{\mathsf{s}}} 
\newcommand{\smin}{\ensuremath{\mathsf{s}_{\sf min}}}
\newcommand{\smax}{\ensuremath{\mathsf{s}_{\sf max}}}
\newcommand{\sgmin}{\ensuremath{\mathsf{s}_{\sf gmin}}}
\newcommand{\sgmax}{\ensuremath{\mathsf{s}_{\sf gmax}}}
\newcommand{\zeroprob}{\ensuremath{\mathsf{p}}} 

\newcommand{\vecbitt}{\ensuremath{\gamma}}


\newcommand{\bitlen}{\ensuremath{{\ell}}}
\newcommand{\error}{\ensuremath{\mathsf{error}}} 

\newcommand{\share}[2]{\ensuremath{{\langle #1 \rangle}_{#2}}}
\newcommand{\shareB}[2]{\ensuremath{{\langle #1 \rangle}_{#2}^{\bf B}}}

%\newcommand{\arval}[1]{\ensuremath{\prescript{}{\sf a}{#1}}}
\newcommand{\arval}[1]{\ensuremath{{#1}^\mathsf{A}}}

%\newcommand{\numshares}{\ensuremath{\mathsf{q}}}
\newcommand{\cset}[1]{\ensuremath{\mathtt{n}\left({#1}\right)}} 
%\newcommand{\shareset}[1]{\ensuremath{\mathsf{P}_{#1}}} 

\newcommand{\maxv}{\ensuremath{\mathsf{max}}} 
\newcommand{\minv}{\ensuremath{\mathsf{min}}} 

\newcommand{\pubconst}{c}

%--------------------------------------------------------------
% System Entities
%--------------------------------------------------------------
\newcommand{\serverset}{\ensuremath{\mathcal{S}}}
\newcommand{\server}[1]{\ensuremath{\mathsf{S}_{#1}}} 
\newcommand{\numservers}{\ensuremath{\tau}} 
%\newcommand{\numservers}{\ensuremath{\mathsf{t}}} 
%\newcommand{\singleserver}{\ensuremath{\mathsf{S}}}
%\newcommand{\serverset}[1]{\ensuremath{\mathbf{P}^{#1}}} 
 

\newcommand{\client}[1]{\ensuremath{\mathsf{C}_{#1}}} 
\newcommand{\numclients}{\ensuremath{\mathsf{n}}} 
\newcommand{\numcoordinates}{\ensuremath{\mathsf{m}}}

\newcommand{\numshares}{\ensuremath{\mathsf{q}}}
\newcommand{\shareset}{\ensuremath{\mathcal{Q}}}

%--------------------------------------------------------------
% Macros for Primitives and Protocols
%--------------------------------------------------------------
\newcommand{\mult}{\ensuremath{\mathsf{Mult}}} 
\newcommand{\dotp}{\ensuremath{\mathsf{DotP}}} 
\newcommand{\pidotp}[2]{\ensuremath{\Pi_\mathsf{mdp}^{#1}(#2)}} 
\newcommand{\bitA}{\ensuremath{\mathsf{Bit2A}}} 
\newcommand{\sbitA}{\ensuremath{\mathsf{SBit2A}}}
\newcommand{\bitinj}{\ensuremath{\mathsf{BitInj}}} 
\newcommand{\sbitinj}{\ensuremath{\mathsf{SBitInj}}}

\newcommand{\bitACost}{\ensuremath{\mathsf{BitA}}} 
\newcommand{\bitAPreCost}{\ensuremath{\mathsf{BitA}^\mathsf{pre}}} \newcommand{\bitAOnCost}{\ensuremath{\mathsf{BitA}^\mathsf{on}}}
\newcommand{\MultCost}{\ensuremath{\mathsf{Mult}}} 
\newcommand{\MultPreCost}{\ensuremath{\mathsf{Mult}^\mathsf{pre}}} \newcommand{\MultOnCost}{\ensuremath{\mathsf{Mult}^\mathsf{on}}}

\newcommand{\truthtable}[1]{\ensuremath{T_{#1}}}

\newcommand{\termSum}{\ensuremath{\mathsf{term_s}}} 
\newcommand{\termMid}{\ensuremath{\mathsf{term_m}}} 
\newcommand{\termProd}{\ensuremath{\mathsf{term_p}}} 
\newcommand{\termMidApx}{\ensuremath{\mathsf{term_m^a}}}

\newcommand{\E}{\ensuremath{\mathds{E}}}
\newcommand{\sampleindices}{\ensuremath{\mathcal{I}}}

%--------------------------------------------------------------
% Macros related to implementation
%--------------------------------------------------------------
\newcommand{\extdecimal}[1]{\textcolor{darkred}{#1}} %2t decimal representation

\newcommand{\svA}[1]{\textcolor{britishracinggreen}{#1}} %Server A
\newcommand{\svB}[1]{\textcolor{darkblue}{#1}} %Server B
\newcommand{\svH}[1]{\textcolor{darkred}{#1}} %Helper
%--------------------------------------------------------------
% Macros for Others
%--------------------------------------------------------------
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\Rebuttal}[1]{\textcolor{blue}{\emph{\textbf{Response:} #1}}}

\newcommand{\rebuttaltitles}[1]{\medskip\noindent{\underline{\emph{#1}}}\smallskip\newline}

\newcommand{\rebuttalsubtitles}[1]{\smallskip\noindent{{\emph{#1:}}}}

\newcommand{\setV}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\hd}{\ensuremath{\mathsf{HD}}}

\DeclareMathOperator*{\argmax}{argmax} % thin space, limits underneath in displays









%Values
\newcommand{\val}{\ensuremath{\mathsf{v}}} 
\newcommand{\vecsize}{\ensuremath{\mathsf{d}}} 
\newcommand{\truncsize}{\ensuremath{\mathsf{f}}}

%Arithmetic Shares
\newcommand{\Mv}[1]{\ensuremath{\mathsf{M}_{#1}}} 
\newcommand{\Lv}[2]{\ensuremath{{\Lambda}_{#1}^{#2}}}
\newcommand{\Gv}[2]{\ensuremath{{\Gamma}_{#1}^{#2}}}

%Boolean Shares
\newcommand{\mv}[1]{\ensuremath{\mathsf{m}_{#1}}} 
\newcommand{\lv}[2]{\ensuremath{{\lambda}_{#1}^{#2}}}
\newcommand{\gv}[2]{\ensuremath{{\gamma}_{#1}^{#2}}}

%Arithmetic Equivalent Shares
%\newcommand{\mvA}[1]{\ensuremath{\tilde{\mathsf{m}}_{#1}}} 
%\newcommand{\lvA}[2]{\ensuremath{{\tilde{\lambda}}_{#1}^{#2}}}

%Sharing Schemes
\newcommand{\sqr}[1]{\ensuremath{[#1]}}
\newcommand{\sqrB}[1]{\ensuremath{[#1]^{\bf B}}}
\newcommand{\shr}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\shrB}[1]{\ensuremath{\langle #1 \rangle}^{\bf B}}
\newcommand{\shrv}[2]{\ensuremath{\langle #1 \rangle}_{#2}}

%Fields and Rings
\newcommand{\GF}[1]{\ensuremath{\mbox{GF}(2^ #1)}}
\newcommand{\Z}[1]{\ensuremath{\mathbb{Z}}_{2^{#1}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}

%Boolean Ring
\newcommand{\bitb}{\ensuremath{\mathsf{b}}} 

\newcommand{\bitbext}{\ensuremath{\tilde{\mathsf{b}}}} 
\newcommand{\bitbAr}{\ensuremath{\tilde{\mathsf{b}}}} 
%\newcommand{\bitbAr}{\ensuremath{\grave{\mathsf{b}}}} 
\newcommand{\bitbapprox}{\ensuremath{\hat{\mathsf{b}}}} 

\newcommand{\bitB}{\ensuremath{\mathsf{B}}} 
%\newcommand{\bitbA}{\ensuremath{\tilde{\mathsf{b}}}} 
\newcommand{\bitbA}{\ensuremath{\mathsf{B}}} 


%Protocols
\newcommand{\piSh}{\ensuremath{\Pi_{\sf Sh}}} %Input Sharing
\newcommand{\piRec}{\ensuremath{\Pi_{\sf Rec}}} %Output Reconstruction
\newcommand{\piLinComb}{\ensuremath{\Pi_{\sf LC}}} %Linear Combination FPA
\newcommand{\piMult}{\ensuremath{\Pi_{\sf Mult}}} %Multiplication
\newcommand{\piDotP}{\ensuremath{\Pi_{\sf IP}}} %Inner Product
\newcommand{\piDotPre}{\ensuremath{\Pi_{\sf IP}^{\sf Pre}}} %Inner Product Precomputation
\newcommand{\piTr}{\ensuremath{\Pi_{\sf Tr}}} %Truncation Pair
%
\newcommand{\pimult}{\ensuremath{\Pi_{\sf Mult}}}

\newcommand{\piOT}[1]{\ensuremath{\Pi_{\sf OT}^{\sf #1}}} %OT
\newcommand{\daBitPrio}{\mathsf{daBitGen}_{p}}


\newcommand{\piBitA}{\ensuremath{\Pi_{\sf BitA}}} %Bit to Arithmetic
\newcommand{\piBitAPre}{\ensuremath{\Pi_{\sf BitA}^{\sf Pre}}} %Bit to Arithmetic Preprocessing
\newcommand{\piBitInj}{\ensuremath{\Pi_{\sf BI}}} %Bit Injection
\newcommand{\piBitInjPre}{\ensuremath{\Pi_{\sf BI}^{\sf Pre}}} %Bit Injection Pre
\newcommand{\piBitASum}{\ensuremath{\Pi_{\sf BitA}^{\sf sum}}} %Bit to Arithmetic Sum
\newcommand{\piSecAgg}[1]{\ensuremath{\Pi_{\sf SecAgg}^{\text{\Romannum{#1}}}}} %Secure Aggregation
\newcommand{\piSecAggG}{\ensuremath{\Pi_{\sf SecAgg}^{\textsf{Global}}}} %Secure Aggregation Global

%--------------------------------------------------------------
% Macros for Defense
%--------------------------------------------------------------
\newcommand{\normval}[1]{\ensuremath{{\sf L}_{#1}}} %General notation for Norms
\newcommand{\normtwo}[1]{\ensuremath{\normval{2}^{#1}}} %L2 norm
\newcommand{\normtwoC}[1]{\ensuremath{\normval{2}^{\client{#1}}}} %L2 norm for client
\newcommand{\normtwoavg}{\ensuremath{\normval{2}^{\sf avg}}} %L2 norm average
\newcommand{\defthreshold}{\ensuremath{\mu_{\sf th}}}
%\newcommand{\defthreshold}{\ensuremath{\normval{2}^{\sf th}}} %Defense L2 threshold


\newcommand{\rejectlist}{\ensuremath{\mathcal{X}}}


\newcommand{\piDefense}{\ensuremath{\Pi_{\sf Defense}}}%secure aggregation with defense
\newcommand{\ltwoplain}{\ensuremath{\mathsf{L_2}}}%l2
\newcommand{\linfplain}{\ensuremath{\mathsf{L_{\infty}}}}%l_infinity

\newcommand{\clientnorm}[1]{\ensuremath{\mathsf{norm}^{#1}}}%act L2
\newcommand{\clientnormavg}{\ensuremath{\mathsf{norm}^{\sf avg}}}%avg l2
\newcommand{\clientinvnorm}[1]{\ensuremath{\mathsf{inv\mbox{-}norm}^{#1}}}%act L2

\newcommand{\actltwo}{\ensuremath{\mathsf{ActSqL_2}}}%act L2
\newcommand{\avgltwo}{\ensuremath{\mathsf{Avg_{\ltwoplain-norm}}}}%avg l2
\newcommand{\avgMin}{\ensuremath{\mathsf{AvgU}}}%avg min Scale
\newcommand{\avgB}{\ensuremath{\mathsf{AvgV}}}%avg max Scale
\newcommand{\avgUpdate}{\ensuremath{\mathsf{AvgUpdate}}}%avg l2
\newcommand{\normscale}{\ensuremath{\mathsf{Scale_{\ltwoplain}}}}%l2-scale
\newcommand{\cosineComput}{\ensuremath{\mathsf{Comp_{Cos}}}}%cosine distance computation
\newcommand{\cosineSorting}{\ensuremath{\mathsf{Sort_{Cos}}}}%cosine distance based sorting & exclusion
\newcommand{\cosineThreshold}{\ensuremath{\mathsf{Thres_{Cos}}}}%cosine distance based sorting & exclusion
\newcommand{\updatedScaleV}[1]{\ensuremath{\mathsf{\hat{s}}^{#1}}}%scaled scale
\newcommand{\avgCosine}{\ensuremath{\shr{\mathsf{Avg_{cos}}}}}%scaled scale
\newcommand{\std}{\ensuremath{\sigma}}%cosine lower threshold
\newcommand{\uThresCos}{\ensuremath{\mathsf{uThres_{cos}}}}%cosine upper threshold
\newcommand{\lThresCos}{\ensuremath{\mathsf{lThres_{cos}}}}%cosine lower threshold
\newcommand{\adversaryquota}{\ensuremath{\alpha}}%percentage of malicious clients
\newcommand{\filterpercentile}{\ensuremath{\mathsf{filterValue}}}%filter value for percentile


%Ideal functionalities
\newcommand{\FSETUP}{\ensuremath{\mathcal{F}_{\mathsf{setup}}}} %Key Setup Functionality


%
\newcommand{\vlu}{\ensuremath{\mathsf{u}}} 
\newcommand{\vlv}{\ensuremath{\mathsf{v}}} 
\newcommand{\vlw}{\ensuremath{\mathsf{w}}} 
\newcommand{\vlx}{\ensuremath{\mathsf{x}}} 
\newcommand{\vly}{\ensuremath{\mathsf{y}}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mypar}[1]{\textbf{#1.}}
\newcommand{\myparatight}[1]{\smallskip\noindent{\bf {#1}:}~}

\newcommand{\restatableeq}[3]{\label{#3}#2\gdef#1{#2\tag{\ref{#3}}}}


%--------------------------------------------------------------
%User Defined Theorems
%--------------------------------------------------------------
%\newtheorem{terminology}{Terminology}
\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{notation}[theorem]{Notation}
%\newtheorem{openproblem}[theorem]{Open Problem}

\newcommand{\tsparagraph}[1]{\noindent\textbf{#1.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{darkred}{\ding{55}}}%



%--------------------------------------------------------------
%Custom Lists
%--------------------------------------------------------------

\newenvironment{myitemize}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			%\setlength\parsep{0pt}
			\setlength\parsep{2pt}
			\setlength\topsep{4pt}
			\setlength\itemsep{3pt}
			%\setlength\itemsep{2pt}
			\setlength{\itemindent}{15pt}
			\setlength{\leftmargin}{2pt}
		}
	}{
		%\vspace{1mm}
	\end{list}
}

\newenvironment{myenumerate}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			%\setlength\parsep{0pt}
			\setlength\parsep{2pt}
			\setlength\topsep{4pt}
			\setlength\itemsep{3pt}
			%\setlength\itemsep{2pt}
			\setlength{\itemindent}{15pt}
			\setlength{\leftmargin}{2pt}
		}
	}{
		%\vspace{1mm}
	\end{list}
}

\newenvironment{boxenumerate}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			%\setlength\parsep{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{0pt}
			\setlength\itemsep{0pt}
			%\setlength\itemsep{2pt}
			\setlength{\itemindent}{4pt}
			\setlength{\leftmargin}{8pt}
		}
	}{
		%\vspace{1mm}
	\end{list}
}



%--------------------------------------------------------------
%Commands for figures and tables and references
%--------------------------------------------------------------
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}

%--------------------------------------------------------------
%New Style boxes
%--------------------------------------------------------------

%\newcommand{\boxref}[1]{Fig.~\ref{#1}}
\newcommand{\boxref}[1]{Fig.~\ref{#1}}

%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}



%Basic box structure with title box
\newenvironment{titlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\footnotesize]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	%\vspace{-2em} %CCS
	%\vspace{-1.8em} %USENIX/PETS
	\vspace{-1.5em} %NDSS
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\smallskip
	%\vspace{1mm}
}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.5cm, inner sep=2pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]



%box style
\mdfdefinestyle{commonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}


\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[3]
{\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gsystembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{protocolbox}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{algobox}[3]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{reductionbox}[3]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gamebox}[3]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}
	
	
%Filled Variants
\tikzstyle{mygray} = [fill=gray!20, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonboxgray}{%
    tikzsetting={fill=gray!10,fill opacity=0.5},
	align=center, middlelinewidth=1.5pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
}

\mdfdefinestyle{roundboxgray}{
style=commonboxgray,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{protboxgray}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonboxgray}{mygray}{#2}{#3}}
	{\end{titlebox}}
	
\newenvironment{systemboxgray}[3]
{\begin{titlebox}{Functionality \normalfont #1}{roundboxgray}{mygray}{#2}{#3}}
	{\end{titlebox}}
	
\newenvironment{simulatorboxgray}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonboxgray}{mygray}{#2}{#3}}
	{\end{titlebox}}
	
%splitbox style
\mdfdefinestyle{commonsplitboxgray}{%
    tikzsetting={fill=gray!10,fill opacity=0.5},
	align=center, middlelinewidth=1.5pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
}

\mdfdefinestyle{roundboxgray}{
style=commonboxgray,roundcorner=5pt,userdefinedwidth=\linewidth}

\mdfdefinestyle{roundsplitboxgray}{
style=commonsplitboxgray,roundcorner=5pt,userdefinedwidth=\linewidth}
	
\newenvironment{splitprotboxgray}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitboxgray}{mygray}{#2}{#3}}
	{\end{splittitlebox}}
	
\newenvironment{splitsystemboxgray}[3]
{\begin{splittitlebox}{Functionality \normalfont #1}{roundsplitboxgray}{mygray}{#2}{#3}}
	{\end{splittitlebox}}
	
\newenvironment{splitsimulatorboxgray}[3]
{\begin{splittitlebox}{Simulator \normalfont #1}{commonsplitboxgray}{mygray}{#2}{#3}}
	{\end{splittitlebox}}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
%Split Box for IEETran Version
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{splittitlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\footnotesize]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	%\vspace{-1em} %CCS
	%\vspace{-0.8em} %USENIX/PETS
	\vspace{-0.5em} %NDSS
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\smallskip
	%\vspace{-2mm}
}

\mdfdefinestyle{commonsplitbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}

\newenvironment{protocolsplitbox}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}


\newenvironment{simulatorsplitbox}[3]
{\begin{splittitlebox}{Simulator \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}

\newenvironment{systemsplitbox}[3]
{\begin{splittitlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
%------------------------------------------------------------------------------
% Full Width Environments
%------------------------------------------------------------------------------

\newenvironment{systembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gsystembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{protocolbox*}[3]
{\begin{strip}
\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{algobox*}[3]
{\begin{strip}
\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{reductionbox*}[3]
{\begin{strip}
\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gamebox*}[3]
{\begin{strip}
\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{simulatorbox*}[3]
{\begin{strip}
\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}




%------------------------------------------------------------------------------
%Basic box structure with mytitle box without embossed title
%------------------------------------------------------------------------------

%box style
\mdfdefinestyle{mycommonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=3pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
}
\mdfdefinestyle{myroundbox}{style=mycommonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{titlebox*}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=0.3\baselineskip,
		skipabove={0.4em},
		skipbelow={1em},needspace=3\baselineskip,
		frametitleaboveskip=5em,
		innerrightmargin=5pt
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.2em}
	{\captionof{figure}{\normalfont \TitleCaption}\label{\TitleLabel}}
	%\medskip
	%\vspace{-2mm}
}

%------------------------------------------------------------------------------
% Box Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox}[3]
{\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygsystembox}[3]
{\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myprotocolbox}[3]
{\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myalgobox}[3]
{\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myreductionbox}[3]
{\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygamebox}[3]
{\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mysimulatorbox}[3]
{\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}
%-------------------------------------------------------------------------------


%------------------------------------------------------------------------------
% Full Width Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygsystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myprotocolbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myalgobox*}[3]
{\begin{strip}
		\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myreductionbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygamebox*}[3]
{\begin{strip}
		\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mysimulatorbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}



%-------------------------------------------------------------------------------
% Basic protocol box without Algohead NDSS
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{mytbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	%\vspace{-2em} %CCS
	%\vspace{-1.8em} %USENIX/PETS
	\vspace{-1.5em} %NDSS
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\smallskip
	%\vspace{-2mm}
}

\newenvironment{mytsplitbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\smallskip
	%\vspace{-2mm}
}

\newenvironment{mypbox}[3]
{\begin{mytbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytbox}}

\newenvironment{mypsplitbox}[3]
{\begin{mytsplitbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytsplitbox}}

%-------------------------------------------------------------------------------
% Macros used for the examples
%-------------------------------------------------------------------------------

%----- Algorithm Environment ---------------------------------------------------
%Header for Algorithms/Functionalities
%\newcommand{\algoHead}[1]{\vspace{-3pt} \underline{\textbf{#1}} \vspace{-1em}} %PETS
%\newcommand{\algoHead}[1]{\vspace{-3pt} \underline{\textbf{#1}} \vspace{-3pt}} %NDSS23
\newcommand{\algoHead}[1]{\vspace{-1pt} \underline{\textbf{#1}} \vspace{-1pt}}
\newcommand{\algoHeadN}[1]{\vspace{-1em} \underline{\textbf{#1}} \vspace{0.2em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}

%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
	\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother

%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}

%  Font and Notation
%-------------------------------------------------------------------------------
\newcommand{\xmath}[1]{\ensuremath{#1}\xspace}

\newcommand{\command}[1]{\xmath{\textsc{#1}}}
%\newcommand{\algorithm}[1]{\xmath{\mathsf{#1}}}
\newcommand{\variable}[1]{\xmath{\mathtt{#1}}}
\newcommand{\parameter}[1]{\xmath{\mathtt{#1}}}

%Nice empty set
\let\oldemptyset\emptyset
\let\emptyset\varnothing

%Functionalities
\newcommand{\Func}[1][\relax]{\xmath{\mathcal{F}_{\textsc{#1}}}}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
% Macros for lists
%-------------------------------------------------------------------------------


%To remove the left indentation of description environment
\setlist[description]{style=unboxed,leftmargin=0cm}
